Code Shaping: Iterative Code Editing with Free-form AI-Interpreted Sketching

We introduce the concept of code shaping, an interaction paradigm for editing code using free-form sketch annotations directly on top of the code and console output. To evaluate this concept, we conducted a three-stage design study with 18 different programmers to investigate how sketches can communicate intended code edits to an AI model for interpretation and execution. The results show how different sketches are used, the strategies programmers employ during iterative interactions with AI interpretations, and interaction design principles that support the reconciliation between the code editor and sketches. Finally, we demonstrate the practical application of the code shaping concept with two use case scenarios, illustrating design implications from the study.

==> tables/anova-results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}

% macros for sig asterisk and spce
% \newcommand{\sig}[0] { \textasteriskcentered\hspace{1.0pt} }
\newcommand{\tabspacelg}{\vspace{0.8em}}
\newcommand{\tabspacesm}{\vspace{0.25em}}

% \newcommand{\tabletab}{\hspace{1em}}

% \newcommand{\ns}[0] { \hspace{3.6pt} }

\small
\begin{tabular}{@{}llrrl@{}}



\toprule
% main effect  
\multicolumn{5}{l}{\tabspacesm (a) \f{tech} (\anova{2}{46}{31.45}{.0001}{0.47})} \\ 
% post hoc tests
\multicolumn{2}{l}{\textit{comparisons} } & \textit{diff (ms)} & \multicolumn{2}{l}{\textit{p-value}}   \\ 
\midrule
\f{cooltech} & \f{supertouch} & 234  & .014 & * \\ 
\f{cooltech} & \f{baseline} & 500  & < .0001 & *** \\ 
\f{supertouch} & \f{baseline} & -123  & .23 &  \tabspacelg \\ 

% interaction  

% \toprule
\multicolumn{5}{l}{\tabspacesm  (b) \f{tech} \by{} \f{task} (\anova{2}{46}{31.45}{.0001}{0.47})} \\ 
% interaction group post hoc tests
\multicolumn{2}{l}{\textit{comparisons for} \f{tapping} } & \textit{diff (ms)} & \multicolumn{2}{l}{\textit{p-value}}   \\                      \midrule
\f{cooltech} & \f{supertouch} & 234  & .014 & * \\ 
\f{cooltech} & \f{baseline} & 500  & < .0001 & *** \\
\f{supertouch} & \f{baseline} & -123  & .23 &  \tabspacesm \\ 
% interaction group post hoc tests
\multicolumn{2}{l}{\textit{comparisons for} \f{dragging} } & \textit{diff (ms)} & \multicolumn{2}{l}{\textit{p-value}}   \\                      \midrule
\f{cooltech} & \f{supertouch} & 234  & .014 & * \\ 
\f{cooltech} & \f{baseline} & 500  & < .0001 & *** \\ 
\f{supertouch} & \f{baseline} & -123  & .23 &   \\ 
\bottomrule

\end{tabular}

